Some facts about the optimality of the LSE in the Gaussian sequence model with convex constraint

We consider a convex constrained Gaussian sequence model and characterize necessary and sufficient conditions for the least squares estimator (LSE) to be minimax optimal. For a closed convex set $K\subset \mathbb{R}^n$ we observe $Y=\mu+\xi$ for $\xi\sim \mathcal{N}(0,\sigma^2\mathbb{I}_n)$ and $\mu\in K$ and aim to estimate $\mu$. We characterize the worst case risk of the LSE in multiple ways by analyzing the behavior of the local Gaussian width on $K$. We demonstrate that optimality is equivalent to a Lipschitz property of the local Gaussian width mapping. We also provide theoretical algorithms that search for the worst case risk. We then provide examples showing optimality or suboptimality of the LSE on various sets, including $\ell_p$ balls for $p\in[1,2]$, pyramids, solids of revolution, and multivariate isotonic regression, among others.

==> main_sections/funding.tex <==
\section{Funding}

The authors report no financial conflicts of interest.

==> main_sections/main_results_algorithms_IEEE_version.tex <==

\section{Algorithms searching for the worst case rate of the LSE on bounded sets} \label{section:algorithm_proofs}


 The results of Section \ref{subsection:characterizations:conditions:worst:case}, in particular Theorems \ref{big:width:minus:small:width:thm} and \ref{difference:of:local:widths:compared:to:eps:squared:thm}, inspire theoretical algorithms for searching for worst case rate for the LSE for bounded sets $K$. Our Algorithm \ref{algo_local_packing} below is based on local packings while Algorithm \ref{algo_global_packing} instead uses global packings. Since both algorithms make usage of evaluating the map $\nu \mapsto w_{\nu}(\varepsilon)$, before we introduce them we will illustrate how one can evaluate the map $\nu \mapsto w_\nu(\varepsilon)$ on a given closed convex body $K$, where it is assumed that we have a separation oracle for $K$. A separation oracle for $K$ is a function $\cO_K\colon\RR^n\to\RR^n$ such that $\cO_K(\nu) = 0$ if $\nu \in K$ and if $\nu\not\in K$,  $\cO_K(\nu) = a$ where $a \in \RR^n$  is such that $a\T \nu > a\T \mu$ for all points $\mu \in K$. The next lemma states that if one can compute the LSE for $K$, then assuming a separation oracle for $K$ is not a stringent assumption.
\begin{lemma}\label{sep:oracle:with:projection}
    If one can project on $K$, i.e., one can calculate $\Pi_K\nu$ for any $\nu \in \RR^n$, then one has a separation oracle on $K$.
\end{lemma}

\begin{proof}
Define $\cO_K(\nu) = \nu - \Pi_K \nu$ for all $\nu\in\RR^n$. Then $\cO_K(\nu)=0$ for all $\nu \in K$. If $\nu\not\in K$, observe that for any  $\mu \in K$ we have $(\nu - \Pi_K \nu)\T (\nu - \mu) > 0$. This follows by \citet[equation (1.19)]{bellec2018sharp} since \begin{align*}
    (\nu - \Pi_K \nu)(\mu - \nu) + \|\nu - \Pi_K \nu\|^2 &= (\nu - \Pi_K \nu)\T (\mu - \Pi_K(\nu)) \\ &\leq 0,
\end{align*} and also that $\|\nu - \Pi_K \nu\| > 0$ since $\nu\not\in K$.
\end{proof}

The idea for calculating the width $w_\nu(\varepsilon)$ is simple, and we summarize it in Algorithm \ref{algo_gaussian_width}. We will sample $N$ points $\xi_i \sim \cN(0,\II_n)$, $i \in [N]$. Assume for a moment we can calculate the values of $\sup_{\eta \in B(\nu,\varepsilon)\cap K} \langle \xi_i, \eta - \nu \rangle $. We will then average all these values as an estimate of $w_\nu(\varepsilon)$. This strategy works because of the celebrated concentration inequality of Lipschitz functions of Gaussian variables \citep[e.g.,][Theorem 2.26]{wainwright2019high}, noting that the map $x \mapsto \sup_{\eta \in B(\nu,\varepsilon)\cap K} \langle x, \eta -\nu\rangle $ is $\varepsilon$-Lipschitz \citep[see][Example 2.30]{wainwright2019high}. The concentration result states that $\langle \xi_i, \eta^*_i -\nu\rangle$ (where $\eta^*_i$ denotes the maximum of $\sup_{\eta \in B(\nu,\varepsilon)\cap K} \langle \xi_i, \eta  -\nu \rangle$) is a sub-Gaussian random variable with variance proxy $\varepsilon^2$, hence satisfies
\begin{align*}
    \PP\bigg(\big|N^{-1}\sum_{i \in [N]} \langle \xi_i, \eta^*_i  -\nu \rangle - w_\nu(\varepsilon)\big| \geq t\bigg) \leq 2 \exp\left(-\frac{Nt^2}{2\varepsilon^2}\right).
\end{align*}
Thus if one wants to approximate $ w_\nu(\varepsilon)$ to precision $t$ with probability at least $1 - \delta$, then one needs at most $N = 2\varepsilon^2\log(2/\delta)/t^2$ observations.

To solve $\sup_{\eta \in B(\nu,\varepsilon)\cap K} \langle \xi_i, \eta - \nu \rangle $ for a fixed $\xi$ given a separation oracle for $K$, we use the ellipsoid algorithm \citep[Chapter 3]{grotschel_ellipsoid}. At each iteration, we must either find a separation oracle for $B(\nu, \varepsilon)$ (which is trivial by Lemma \ref{sep:oracle:with:projection}), or a separation oracle for $K$. If the point $\eta$ happens to be in the set $B(\nu,\varepsilon) \cap K$ then one simply needs to take the gradient of $-\langle\xi, \eta -\nu \rangle$ with respect to $\eta$ which is also trivial. 

% \begin{algorithm}
% \SetKwComment{Comment}{/* }{ */}
% \caption{Local Gaussian Width Algorithm}\label{algo_gaussian_width}
% \KwInput{$K$ a compact convex set in $\RR^n$, a separation oracle $\cO_K$ for $K$, a point $\nu\in K$, $\varepsilon>0$, desired precision $t$ and probability $1-\delta$.}
% Let $\cE$ be a subroutine that can solve $\arg\sup_{\eta\in B(\nu, \varepsilon)\cap K}\langle \xi,\eta-\nu\rangle$ given $\cO_K$\;
% Set $N = \lceil 2\varepsilon^2 \log(2/\delta)/t^2\rceil$\;
% Draw $\xi_1,\dots,\xi_N \sim \cN(0,\II_n)$ \;
% Compute using $\eta_i^{\ast}=\arg\sup_{\eta\in B(\nu, \varepsilon)\cap K}\langle \xi_i,\eta - \nu\rangle$ for $i=1,\dots,N$ using $\cE$\;
% Set $\widehat{w_{\nu}}(\varepsilon) = N^{-1}\sum_{i\in[N]}\langle \xi_i, \eta_i^{\ast} - \nu\rangle$\;
% \Return{$\widehat{w_{\nu}}(\varepsilon)$}  
% \end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}
\caption{Local Gaussian Width Algorithm}\label{algo_gaussian_width}
\STATE {\textsc{INPUT}} $K$ a compact convex set in $\RR^n$, a separation oracle $\cO_K$ for $K$, a point $\nu\in K$, $\varepsilon>0$, desired precision $t$ and probability $1-\delta$.
\STATE Let $\cE$ be a subroutine that can solve $\arg\sup_{\eta\in B(\nu, \varepsilon)\cap K}\langle \xi,\eta-\nu\rangle$ given $\cO_K$
\STATE Set $N = \lceil 2\varepsilon^2 \log(2/\delta)/t^2\rceil$
\STATE Draw $\xi_1,\dots,\xi_N \sim \cN(0,\II_n)$ 
\STATE Compute using $\eta_i^{\ast}=\arg\sup_{\eta\in B(\nu, \varepsilon)\cap K}\langle \xi_i,\eta - \nu\rangle$ for $i=1,\dots,N$ using $\cE$
\STATE Set $\widehat{w_{\nu}}(\varepsilon) = N^{-1}\sum_{i\in[N]}\langle \xi_i, \eta_i^{\ast} - \nu\rangle$
\RETURN $\widehat{w_{\nu}}(\varepsilon)$
\end{algorithmic}
\end{algorithm}  

\subsection{A local packing algorithm}



% \begin{algorithm}[t]
% \SetKwComment{Comment}{/* }{ */}
% \caption{Local Packing Algorithm}\label{algo_local_packing}
% \KwInput{Compact convex set $K$, diameter $d$,  constant $c^{\ast}$ from definition of local metric entropy}
% \SetKwFunction{ChildrenDistance}{ChildrenDistance}
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\ChildrenDistance{$\nu\in K$, $k\in\NN$}}{
%   $\delta\gets\frac{d}{2^{k-1}c^{\ast}}$\;
%     Form a maximal $\delta$-packing set $\{\nu_1^k,\nu_2^k, \dots,\nu_M^k\}$ of the set $B(\nu,\delta c^{\ast})\cap K$ where $M=\cM(\delta, B(\nu,\delta c^{\ast})\cap K)$\; 
%     Solve $\nu_i^{k\ast} = \argmin_i w_{\nu_i^k}(\delta)$\;
%     $\Psi \gets w_{\nu}(\delta c^{\ast}) - w_{\nu_i^{k\ast}}(\delta)$\; 
%     $T\gets C(\delta c^{\ast})^2/(2\sigma$)\;
%     \KwRet{$\Psi - T$}\;
%   }
%   Initialize $\nu^{\ast}\in K$\;
%   Set $\phi(\nu^{\ast})=1$ \tcc*{Track the level of any node $\nu$ in the tree}
%   Let $Q=(\nu^{\ast})$ be an ordered queue\;
% \While{$Q$ is not empty}{
%     Remove the point $\nu$ at the end of the $Q$\;
%     Compute $\gamma= $ \ChildrenDistance{$\nu$, $\phi(\nu)$} and the packing set therein\;
%     Define $\beta=\dfrac{d}{2^{\phi(\nu)-1}c^*}$\;
%     \uIf{$\gamma> 0$}{
%     \Return{$\beta$}  
%     }
%     \Else{
%     For each child node $\nu_i$ in the packing set, set $\phi(\nu_i)=\phi(\nu)+1$\;
%     Add each $\nu_i$ to the start of $Q$\;
%     }
% }
% % Don't need final return statement as this While loop
% % eventually terminates, i.e., gamma > 0
% \end{algorithm}

\begin{algorithm}[H]
\caption{Local Packing Algorithm}\label{algo_local_packing}
\begin{algorithmic}
\STATE {\textsc{INPUT}} Compact convex set $K$, diameter $d$,  constant $c^{\ast}$ from definition of local metric entropy
\STATE {\textbf{procedure}} {\textsc{ChildrenDistance}}($\nu\in K$, $k\in\NN$)
  \STATE $\delta\gets\frac{d}{2^{k-1}c^{\ast}}$
  \STATE Form a maximal $\delta$-packing set $\{\nu_1^k,\nu_2^k, \dots,\nu_M^k\}$ of the set $B(\nu,\delta c^{\ast})\cap K$ where $M=\cM(\delta, B(\nu,\delta c^{\ast})\cap K)$
   \STATE  Solve $\nu_i^{k\ast} = \argmin_i w_{\nu_i^k}(\delta)$
   \STATE  $\Psi \gets w_{\nu}(\delta c^{\ast}) - w_{\nu_i^{k\ast}}(\delta)$ 
   \STATE $T\gets C(\delta c^{\ast})^2/(2\sigma$)
    \RETURN $\Psi - T$
  \STATE {\textbf{end procedure}} 
  \STATE Initialize $\nu^{\ast}\in K$
  \STATE Set $\phi(\nu^{\ast})=1$ \COMMENT{Track the level of any node $\nu$ in the tree}
  \STATE Let $Q=(\nu^{\ast})$ be an ordered queue
\WHILE{$Q$ is not empty}
      \STATE Remove the point $\nu$ at the end of the $Q$
      \STATE Compute $\gamma= \textsc{ChildrenDistance}(\nu,\phi(\nu))$ and the packing set therein
      \STATE Define $\beta=\dfrac{d}{2^{\phi(\nu)-1}c^*}$
    \IF{$\gamma> 0$}
    \STATE Return $\beta$ 
    \ELSE
    \STATE For each child node $\nu_i$ in the packing set, set $\phi(\nu_i)=\phi(\nu)+1$
    \STATE Add each $\nu_i$ to the start of $Q$\;
    \ENDIF
    \ENDWHILE
% Don't need final return statement as this While loop
% eventually terminates, i.e., gamma > 0
\end{algorithmic}
\end{algorithm}



Suppose $K$ is a compact convex set with diameter $d$. Take $c^{\ast}>4$ in the definition of the local metric entropy, and set $C = 4 - \frac{1}{{c^{\ast}}^2}$. We now consider partitioning $K$ in the following way. Begin by fixing an arbitrary point $\nu^* \in K$ (its location is inconsequential). Maximally pack the set $B(\nu^*, d)\cap K = K$ at a distance $d/c^{\ast}$. Next, for each point  $\nu_i^*$ in that packing set, consider maximally packing the set $B(\nu_i^*, d/2) \cap K$ at a distance $d/(2c^{\ast})$. Continue the process infinitely, obtaining an infinite tree of packing sets. At the $k$th level, the number of descendants of a point from the $(k-1)$th level is bounded by $\cMloc(d/2^{k-1})$. 

Following this packing set construction, we proceed with our algorithm starting with level $k=1$. Algorithm \ref{algo_local_packing} considers the difference between $w(B(\nu^*, d/2^{k-1})\cap K)$ and the smallest possible point from the children of $\nu^*$, i.e., $\min_{i} w(B(\nu_i^*, d/(2^{k-1}c^{\ast})) \cap K)$. If that difference is bigger than $C d^2/(2\sigma)$ then the algorithm stops and outputs $d/c^{\ast}$. If not, it proceeds to look at all children of $\nu^*$ in the same way but replacing $d$ with $d/2$. For example, if we take $\nu_i^*$ the algorithm looks at the difference between $w(B(\nu^*_i, d/2^{2-1})\cap K)$ and the smallest possible difference from its children. If the algorithm finds a point whose corresponding difference exceeds $C (d/2)^2/(2\sigma)$, the algorithm terminates and outputs $d/(2c^{\ast})$. Else, it continues to look at the children of children, and so on, in a breadth-first search manner.



The following theorem (which uses Lemma \ref{lemma:local:packing:algorithm} in the Appendix) states our resulting bounds on $\epsLSE(\sigma)$ depending on how many iterations it takes for the algorithm to terminate.


\begin{theorem} \label{theorem:local:packing:algorithm} Define $c' =\frac{(2c^{\ast}-4)(4c^{\ast}-1/c^{\ast})}{(c^{\ast}-4)c^{\ast}}$ for some $c^{\ast}>4$. \renewcommand\labelenumi{(\theenumi)} 
\renewcommand{\theenumi}{\roman{enumi}}
\begin{enumerate}
    \item  Suppose Algorithm \ref{algo_local_packing} terminates after $k$ iterations. Then $\epsLSE(\sigma) \gtrsim d/(2^{k-1}c^{\ast})$.
    \item Suppose Algorithm \ref{algo_local_packing} does not terminate within $k$ iterations.
        \begin{enumerate}
            \item  If $\sigma \ge c'\cdot \frac{d}{2^k}$, then $\epsLSE(\sigma)\asymp \sigma\wedge d$.
            \item  If $\sigma \le c'\cdot \frac{d}{2^k}$, then  $\epsLSE(\sigma) \lesssim c'\cdot \frac{d}{2^k}$.
        \end{enumerate}
\end{enumerate}
\end{theorem}

\subsection{A global packing algorithm}

In this subsection, we present a global packing algorithm based on Theorem \ref{difference:of:local:widths:compared:to:eps:squared:thm}. We use the same absolute constants $L,c^{\ast},$ and $C$ from the theorem. For a fixed $\sigma>0$, Algorithm \ref{algo_global_packing} (if it does not immediately terminate) produces an $\varepsilon$ that will either match $\epsLSE$ or upper bound it. The algorithm accomplishes this by repeatedly forming $\delta$-packing sets of $K$ with $\delta=\left(\varepsilon^3/(4c^{\ast}\sup_{\eta \in K} w_\eta(\varepsilon/c^{\ast})\sigma) \right)\wedge \varepsilon$, and doubling $\varepsilon$ until a certain condition is met.

% \begin{algorithm}[t]
% \SetKwComment{Comment}{/* }{ */}
% \caption{Global Packing Algorithm}\label{algo_global_packing}
% \KwInput{$K$ a convex set, $\sigma>0$, absolute constants $c^{\ast},L>0$, and $C=8+8/c^{\ast}$.}
% Initialize $\varepsilon \gets 2 \underline\varepsilon^{\ast}$ where $\underline\varepsilon^{\ast}$ is defined in \eqref{underline:varepsilon:def}\;
% $\delta\gets\varepsilon^3/(4c^{\ast}\sup_{\eta \in K} w_\eta(\varepsilon/c^{\ast})\sigma) \wedge \varepsilon$\;
% Form a maximal $\delta$-packing set $\{\nu_1, \nu_2,\ldots, \nu_M\}$ of $K$, where $M = \cM(\delta,K)$\;
% $\Psi\gets \max_{i \in [M]} \sup_{\nu' \in B(\nu_i, 2\varepsilon-\delta)\cap K} w_{\nu'}(\varepsilon/c^{\ast}) - w_{\nu_i}(\varepsilon/c^{\ast})$\;
% $T\gets  C \varepsilon^2/(2\sigma) -( L/c^{\ast})\cdot\varepsilon \sqrt{\log \cMKloc(\varepsilon)}$\;
% \While{$\Psi\ge T$}{
%  $\varepsilon\gets 2\varepsilon$\;
%  Update $\delta$\; 
% Update maximal $\delta$-packing set $\{\nu_1,\dots,\nu_M\}$ of $K$ with $M=\cM(\delta, K)$\;
%  Update $\Psi$ and $T$\;
% }
% \Return{$\varepsilon$}  
% \end{algorithm}

\begin{algorithm}[H]
\caption{Global Packing Algorithm}\label{algo_global_packing}
\begin{algorithmic}
\STATE {\textsc{INPUT}} $K$ a convex set, $\sigma>0$, absolute constants $c^{\ast},L>0$, and $C=8+8/c^{\ast}$.
\STATE Initialize $\varepsilon \gets 2 \underline\varepsilon^{\ast}$ where $\underline\varepsilon^{\ast}$ is defined in \eqref{underline:varepsilon:def}
$\delta\gets\varepsilon^3/(4c^{\ast}\sup_{\eta \in K} w_\eta(\varepsilon/c^{\ast})\sigma) \wedge \varepsilon$
\STATE Form a maximal $\delta$-packing set $\{\nu_1, \nu_2,\ldots, \nu_M\}$ of $K$, where $M = \cM(\delta,K)$
\STATE $\Psi\gets \max_{i \in [M]} \sup_{\nu' \in B(\nu_i, 2\varepsilon-\delta)\cap K} w_{\nu'}(\varepsilon/c^{\ast}) - w_{\nu_i}(\varepsilon/c^{\ast})$
\STATE $T\gets  C \varepsilon^2/(2\sigma) -( L/c^{\ast})\cdot\varepsilon \sqrt{\log \cMKloc(\varepsilon)}$
\WHILE{$\Psi\ge T$}
 \STATE $\varepsilon\gets 2\varepsilon$
 \STATE Update $\delta$\
 \STATE Update maximal $\delta$-packing set $\{\nu_1,\dots,\nu_M\}$ of $K$ with $M=\cM(\delta, K)$
 \STATE Update $\Psi$ and $T$
\ENDWHILE
\RETURN $\varepsilon$
\end{algorithmic}
\end{algorithm}

In computing $\Psi$ from the algorithm, we must solve the problem $\sup_{\nu' \in K\cap B(\nu_i, 2\varepsilon-\delta)} w_{\nu'}(\varepsilon/c^{\ast})$ for each $i$. This is a maximization of a concave function over a convex set and in principle is computationally tractable.

Our main result is stated in Theorem \ref{theorem:global:packing:algorithm}, which relates the output $\varepsilon$ of Algorithm \ref{algo_global_packing}  to $\epsLSE(\sigma)$. The proof uses Lemma \ref{lemma:global:algorithm} to compare $\varepsilon$ to $\epsSupwidth(\sigma)$, and that lemma in turn relies on Lemma \ref{lemma:technical:global:algorithm} to  bound $\varepsilon$ depending on whether $\Psi < T$ or $\Psi \ge T$ (the algorithm's stopping conditions).


\begin{theorem} \label{theorem:global:packing:algorithm} Suppose Algorithm \ref{algo_global_packing} does not terminate on initialization, and let $\varepsilon$ be the output of the algorithm. Then the following hold:
\renewcommand\labelenumi{(\theenumi)} 
\renewcommand{\theenumi}{\roman{enumi}}
\begin{enumerate}
    \item If $d \lesssim \sigma$, then $\epsLSE(\sigma)\asymp d \lesssim \varepsilon$. 
    \item  If $d \gtrsim \sigma$ and $\sigma\ge \varepsilon$, then $\varepsilon\asymp\epsLSE(\sigma)\asymp \sigma\wedge d$. 
    \item If $d\gtrsim \sigma$ and $\sigma\le \varepsilon$, we have $\varepsilon\asymp\epsLSE(\sigma)$. 
\end{enumerate}
If Algorithm \ref{algo_global_packing} does terminate on initialization, $\varepsilon \asymp \epsLSE(\sigma)$. 
\end{theorem}


